Fundamental Limits of Distributed Optimization over Multiple Access Channel

We consider distributed optimization over a $d$-dimensional space, where $K$ remote clients send coded gradient estimates over an {\em additive Gaussian Multiple Access Channel (MAC)} with noise variance $\sigma_z^2$. Furthermore, the codewords from the clients must satisfy the average power constraint $P$, resulting in a signal-to-noise ratio (SNR) of $KP/\sigma_z^2$. In this paper, we study the fundamental limits imposed by MAC on the {convergence rate of any distributed optimization algorithm and design optimal communication schemes to achieve these limits.} Our first result is a lower bound for the convergence rate, showing that communicating over a MAC imposes a slowdown of $\sqrt{d/\frac{1}{2}\log(1+\SNR)}$ on any protocol compared to the centralized setting. Next, we design a computationally tractable {digital} communication scheme that matches the lower bound to a logarithmic factor in $K$ when combined with a projected stochastic gradient descent algorithm. At the heart of our communication scheme is carefully combining several compression and modulation ideas such as quantizing along random bases, {\em Wyner-Ziv compression}, {\em modulo-lattice decoding}, and {\em amplitude shift keying.} We also show that analog schemes, which are popular due to their ease of implementation, can give close to optimal convergence rates at low $\SNR$ but experience a slowdown of roughly $\sqrt{d}$ at high $\SNR$.

==> ratq.tex <==
\newpage
%%% commenting out the subsampling idea- ambigous in combining with Wyner-Ziv idea.
\subsubsection{Based on subsampling and uniform quantization}
\paragraph{Subsampling} In iteration $t$, a subset $S_t\subseteq [d]$ of coordinates is chosen uniformly such that $|S|=p.$
\paragraph{Uniform Quantization}
Each client $k\in \cC_1$ first divides the gradient estimate $\hat{g}_{t,k}$ by $K$ to form $\tilde{g}_{t,k}:=\frac{\hat{g}_{t,k}}{K}$ and quantizes the coordinates in $S_t$ using the $v$-level CUQ defined above in \eqref{e:CUQ}.  All the other coordinates are assigned 0.

Clearly, the CUQ output can be expressed as \[Q_v(\tilde{g}_{t,k}(i))=-\frac{B}{K}+z_{t,k}(i)\frac{2B}{K(v-1)},\qquad i\in S_t,\] where $z_{t,k}(i)\in \{0,\dots, v-1\}.$
\paragraph{Mapping to ASK} Each client $k$ encodes $\{z_{t,k}(i)\}_{i\in S_t}$ and transmit it using an ASK codeword in single channel use. Each of these $z_{t,k}(i)$s are represented using the bases $\{w_2^0, w_2^{p-1}\}$ and is given by 
\[\tau_{t,k}:=z_{t,k}(S_t(1))+\dots+w^{p-1}z_{t,k}(S_t(p)),\]
where $w_2=K(v-1)+1.$
Further, the communication happens over the MAC channel using ASK code in \eqref{e:ASK}.
Specifically,  the encoded output for client $k$ is given by $C_{t,k}=-\sqrt{P} +\frac{\tau_{t,k}\cdot 2\sqrt{P}}{2^r-1}.$ 
 
 Finally,  the corresponding output $Y_{t,\MAC}\in \R$ received is
\[Y_{t,\MAC}(j)=\sum_{k\in \cC_1} \varphi_k(\hat{g}_{t,k})(j)+W_{t}(j), \qquad  1\leq j\leq d/p.\]
%For each block $j\in d/p$, the side information is formed by taking the average of the quantized outputs from all 
\paragraph{Successive cancellation decoding}
At the algorithm's end, the overall decoding function
$\psi$
%consists of three components, namely the minimum-distance decoder,  an inverse mapping $\Omega: [-K\sqrt{P}, K\sqrt{P}]\to \{0,\dots, K(M^d-1)\},$ MQ decoder $\Qdec_{\tt M}$ and inverse rotation, and 
performs the following steps:
\begin{enumerate}
\item The $Y_{t,\MAC}$ is first fed into a minimum-distance (MD) decoder that locates the nearest possible ASK codeword in $[-K\sqrt{P}, K\sqrt{P}]$. Denote the decoded output by $\hat{Y}_{t,\mathtt{MD}}$,
%Note that there exist a one-to-one mapping between the decoded codeword to $$
it is mapped back to the lattice formed by the bases: $\{w_2^0,\dots, w_2^{p-1}\}$ via a mapping $\Omega:[-K\sqrt{P}, K\sqrt{P}]\to \{0,\dots, w^p-1\}$
% \snote{not $K(w^p-1)$ in range of $\Omega$ as maximum is something else} 
given by $\Omega(x)=\frac{x+(K)\sqrt{P}}{2\sqrt{P}/(2^r-1)}.$
{Under perfect decoding, $\Omega(\hat{Y}_{t,\mathtt{MD}})=\sum_{k\in \cC_1}\tau_{t,k}$.}
\item Note that every output $\Omega(\hat{Y}_{t,\mathtt{MD}})$ can be expressed as 
\[\Omega(\hat{Y}_{t,\mathtt{MD}})=w_2^0\lambda_{1}+\dots+w_2^{p-1} \lambda_{p},\] where %\footnote{Under perfect decoding, $\lambda_{ji}=\sum_{i=1}^KI_{ji.$}
$\lambda_{i}\in \{0,\dots, K(v-1)\}, j\in [d/p], i\in [p].$
{Under perfect decoding $\lambda_{i}=\sum_{k\in \cC_1}z_{t,k}(S_t(i)).$}
\item We then follow the successive-cancellation approach to recover each $\lambda_{i}.$ In particular,  we use the following recursion
\[\lambda_{i}=\frac{\Omega(\hat{Y}_{t,\mathtt{MD}})-\lambda_{1}-\dots-w_2^{i-2}\lambda_{i-1}}{w_2^{i-1}}\mod w_2, \ 1\leq i\leq p.\]
\end{enumerate}
The final output $\psi(Y_{t,\MAC})$ is given by 
\[\psi(Y_{t,\MAC})(S_t(i))=\frac{d}{p}\left(-B+\lambda_{i}\cdot \frac{2B}{K(v-1)}\right), \ 1\leq i\leq p.\] 
The rest of coordinates are assigned 0.

\begin{prop}
Under perfect decoding, we have 
\[\alpha(\pi, \bar{\varphi}, \psi)=\frac{2\sigma^2}{K}+ \frac{8B^2d}{K(v-1)^2}, \ \beta(\pi, \bar{\varphi}, \psi)=0.\]
%\[\left|S_t(i)-\sum_{k\in \cC_1}\tilde{g}_{t,k}(i)\right|\leq \frac{2B}{v-1}.\]
\end{prop}
\begin{proof}It is easy to note that
\[\E{\psi(Y_{t,\MAC})}=\frac{1}{K}\sum_{k\in \cC_1}\hat{g}_{t,k}.\]
From the above scheme,  under perfect decoding we have
\begin{align*}
&\E{\left\|\sum_{i\in [d]}\frac{d}{p}\sum_{k\in \cC_1}Q_v(\tilde{g}_{t,k}(i))e_i\cdot \mathbbm{1}_{\{i\in S_t\}}-\sum_{i\in [d]}\sum_{k\in \cC_1}\tilde{g}_{t,k}(i)e_i\right\|^2}\\
&\leq \E{\left\|\sum_{i\in [d]}\frac{d}{p}\sum_{k\in \cC_1}Q_v(\tilde{g}_{t,k}(i))e_i\cdot \mathbbm{1}_{\{i\in S_t\}}-\sum_{i\in [d]}\frac{d}{p}\sum_{k\in \cC_1}\tilde{g}_{t,k}(i)e_i\cdot \mathbbm{1}_{\{i\in S_t\}}\right\|^2}\\
&\qquad +\E{\left\|\sum_{i\in [d]}\frac{d}{p}\sum_{k\in \cC_1}\tilde{g}_{t,k}(i)e_i\cdot \mathbbm{1}_{\{i\in S_t\}}-\sum_{i\in [d]}\sum_{k\in \cC_1}\tilde{g}_{t,k}(i)e_i\right\|^2}\\
&\leq \frac{d}{p}\cdot \frac{4B^2d}{K(v-1)^2}+\frac{dB^2}{Kp}.
\end{align*}

Further, from \eqref{e:mean_square}, we have $\left\|\sum_{k\in \cC_1}\tilde{g}_{t,k}-\nabla f(x_t)\right\|^2\leq \frac{\sigma^2}{K}.$ 
Using the inequality: $(a+b)^2\leq 2(a^2+b^2),$ the proof is completed.
\end{proof}

\begin{thm}\label{t:SamUQSGD}
 Let $\pi$ be the optimization algorithm described in Algorithm \ref{a:SGD_Q} where $Q_t=\sum_{k\in \cC_1}Q_{\mathtt{sub-}v}(\tilde{g}_{t,k})$ is used to make the PSGD step after the $t$th query. Then,
  for universal constants $c_1$ and $c_2$ and 
 $r=\log(1+\sqrt{\SNR/(KN)})$ such that ${d \geq r \geq c_1\log (Kv)}$, we have

\begin{align*}
&\cE(f, \clientset, \pi, S) \leq  \frac{c_2D}{\sqrt{KN}}\sqrt{\sigma^2 +\left(\frac{4d}{(v-1)^2}+1\right) \frac{dB^2\log (Kv)}{r}}+\frac{DB}{K\sqrt{N}}
+ \frac{L D^2}{N}.
\end{align*}
\end{thm}

\newpage
\snote{Keeping it aside as a placeholder if Wyner-Ziv part becomes clear.}
\subsection{Based on RATQ}
We begin by presenting the convergence  result for the baseline scheme in our setup: the {\tt Parallel SGD} algorithm. In {\tt Parallel SGD}, all clients compress their stochastic gradient estimates to $r$ bits using an efficient quantizer for the Euclidean ball, map it to an $2^r$-ASK code and send it over the MAC channel.

%, which then takes the average of the quantized gradients for the projected gradient descent step.
We choose subsampled RATQ (\cite{mayekar2020ratq}) for this efficient quantizer. We denote by $Q_{\tt RATQ}$ the subsampled version of RATQ using $r$ bits, which is described in \cite[Section 3.5]{mayekar2020ratq}.
RATQ first rotates and then performs a 
{\em tetra-iterated adaptive quantization} using an $v_2$-level uniform quantizer. The quantization is done only for the coordinates indexed in $S_t\subset [d], |S_t|=p$, which are sampled uniformly. The output is given by, for some $z_{ik}\in \{0,\dots,v_2-1\},$
\[Q_{\tt RATQ}(\hat{g}_k(x_t))(i)=-M_{ki}^{\ast}+z_{ki}\cdot \frac{2M_{ki}^{\ast}}{v_2-1},\ i\in S_t.\]
Further, $(M_{ki}^{\ast})^2$ is chosen to be the smallest number in the tetra-iterated set
$\mathcal{T}:=\{m, m\cdot e,\dots, m\cdot e^{\ast(h-1)}\}$, defined as $m=\frac{3B^2}{d}, e^{\ast 1}=e, e^{\ast i}=e^{e^{\ast (i-1)}}, \forall i\in [h],$
 such that $|\mathbf{R}\hat{g}_k(x_t)(i)|\leq M_{ki}^{\ast}.$ All the other coordinates are assigned $0.$

Each client $k$ encodes the product $\{z_{ki}M_{ki}^\ast\}_{i\in S_t}$,  and $\{M_{ki}^\ast\}_{i\in S_t}$ separately, and transmit them in two channel uses. In particular, 
let $\mathtt{idp}_{k1}, \dots, \mathtt{idp}_{kp}\in \{0,\dots, h(v_2-1)\}$ be the index corresponding to the product terms $\{z_{ki}M_{ki}^\ast\}_{i\in S_t},$ respectively, and let $\mathtt{id}_{k1}, \dots, \mathtt{id}_{kp}\in \{0,\dots, h-1\}$ be the index corresponding to $\{M_{ki}^\ast\}_{i\in S_t},$ respectively.  Each of these indices are represented using the bases $\{w_2^0,\dots, w_2^{p-1}\}$ 
and are given by
\begin{align*}
\tau_{t,k}&=\begin{bmatrix}
\mathtt{idp}_{k1} & \cdots & \mathtt{idp}_{kp}\\\mathtt{id}_{k1} & \cdots & \mathtt{id}_{kp}
\end{bmatrix}
\begin{bmatrix}
w_2^0\\ 
\vdots \\
w_2^{p-1}
\end{bmatrix},
\end{align*}
where $w_2=Kh(v_2-1)+1$.

Further, the communication happens over the MAC channel, for which, we
consider the following $2^r$-ASK code in $[-\sqrt{P},\sqrt{ P}]$
\begin{align}\label{e:ASK}
\mathcal{B}:=\left\{-\sqrt{P} +\frac{(i-1)\cdot 2\sqrt{P}}{2^r-1}\colon i \in [2^r] \right\},
\end{align}
with $r=p\cdot \log w_2.$
 Specifically,  for client $k$, 
 $\tau_{t,k}$ gets mapped to unique codewords in $\mathcal{B}$ as $C_{t,k}(i)=-\sqrt{P} +\frac{\tau_{t,k}(i) 2\sqrt{P}}{2^r-1}, \ i=1,2.$ 
 
The corresponding output $Y_{t,\MAC}\in \R^{2}$ received is
\[Y_{t,\MAC}=\sum_{k\in \cC_1} C_{t,k}+W_{t}.\]

\paragraph{Successive cancellation decoding}
At the algorithm's end, we perform a coordinate-wise decoding for $Y_{t,\MAC}.$ 
For every coordinate $Y_{t,\MAC}(j)$, the overall decoding function
$\psi$
%consists of three components, namely the minimum-distance decoder,  an inverse mapping $\Omega: [-K\sqrt{P}, K\sqrt{P}]\to \{0,\dots, K(M^d-1)\},$ MQ decoder $\Qdec_{\tt M}$ and inverse rotation, and 
performs the following steps:
\begin{enumerate}
\item Each $Y_{t,\MAC}(j)$ is first fed into a minimum-distance (MD) decoder that locates the nearest possible ASK codeword in $[-K\sqrt{P}, K\sqrt{P}]$. Denote the decoded output by $\hat{Y}_{t,\mathtt{MD}}(j)$,
%Note that there exist a one-to-one mapping between the decoded codeword to $$
it is then passed through a inverse mapping $\Omega:[-K\sqrt{P}, K\sqrt{P}]\to \{0,\dots, w_2^p-1\}$ given by $\Omega(x)=\frac{x+K\sqrt{P}}{2\sqrt{P}/(2^r-1)}.$
{Under perfect decoding, $\Omega(\hat{Y}_{t,\mathtt{MD}}(i))=\sum_{k\in \cC_1}\tau_{t,k}(i), i=1,2$.}
\item Note that every output $\Omega(\hat{Y}_{t,\mathtt{MD}}(j))$ can be expressed as 
\[\Omega(\hat{Y}_{t,\mathtt{MD}}(j))=w^0\lambda_{j1}+\dots+w^{p-1} \lambda_{jp},\] where %\footnote{Under perfect decoding, $\lambda_{ji}=\sum_{i=1}^KI_{ji.$}
$\lambda_{1i}\in \{0,\dots, Kh(v_2-1)\}$ and $\lambda_{2i}\in \{0,\dots, K(h-1)\}, i\in [p].$
{Under perfect decoding $\lambda_{1i}=\sum_{k\in \cC_1}\mathtt{idp}_{ki}$ and $\lambda_{2i}=\sum_{k\in \cC_1}\mathtt{id}_{ki}, \forall i\in [p]$.}
\item We then follow the successive-cancellation approach to recover each $\lambda_{1i}.$ In particular,  we use the following recursion
\[\lambda_{ji}=\frac{\Omega(\hat{Y}_{t,\mathtt{MD}}(j))-\lambda_{j1}-\dots-w^{i-2}\lambda_{j(i-1)}}{w^{i-1}}\mod w, \ 1\leq j\leq d/p,1\leq i\leq p.\]
%which requires the knowledge of previously decoded $\{\hat{\lambda}_{jk}\}_{k=1}^{i-1}.$ To decode these $\lambda_{jk}$ from $\hat{\lambda}_{jk}\mod v,$ we follow the procedure $\Qdec_{\tt M}(\hat{\lambda}_{jk}\mod v)$ described in Algorithm \ref{a:D_MCQ}.

The final output is the side information constructed, i.e.,  $\psi(Y_{t,\MAC})$, and is given by 
\[\psi(Y_{t,\MAC})(i)=-\lambda_{2i}+\lambda_{1i}\cdot \frac{2}{v_2-1}, 1\leq i\leq p.\] 
\end{enumerate}

 Denote by $Q_t$ the average of all the quantized gradients, i.e., 
\begin{align}\label{e:Q_ParSGD}
Q_t=\frac{1}{K}\sum_{i=1}^{K}Q_{\tt RATQ}(\hat{g}_j(x_t)).
\end{align}


We use $Q_t$ to make the projected descent step as seen in line 2 of Algorithm \ref{a:SGD_Q}.
\begin{thm}\label{t:ParSGD}
 Let $\pi$ be the optimization algorithm described in Algorithm \ref{a:SGD_Q} where $Q_t$ as described in \eqref{e:Q_ParSGD} is used to make the PSGD step after the $t$th query. Then,
  for universal constants $c_1$ and $c_2$ and 
 $r=\log(1+\sqrt{\SNR/(KN)})$ such that ${d \geq r \geq c_1\log(K\ln^\ast d)}$, we have
%For optimization domain $\X$ with Euclidean diameter atmost $D$, $(f, \clientset) \in \cO$,  and  $r$ such that ${d \geq r \geq 3+ \ceil{\log(1+ \ln^\ast(d/3))}}$,  Algorithm \ref{a:ParSGD} satisfies the following convergence guarantees:
\begin{align*}
&\cE(f, \clientset, \pi, S) \leq  \frac{c_2D}{\sqrt{KN}}\sqrt{\sigma^2 +\frac{c_2 d B^2 \log (K\ln^\ast d)}{r} }
+ \frac{L D^2}{T}.
\end{align*}

\end{thm}


\subsubsection{The Wyner-Ziv type estimate}
\paragraph{Rotated Modulo quantization}
For a client $k\in \cC_2$,  the gradient estimate $\hat{g}_{t,k}$ is first divided by $K/2$ to form $\tilde{g}_{t,k}:=\frac{\hat{g}_{t,k}}{K/2}.$ 
 \begin{prop}
 For any $\Delta^\prime>0,$ if $|\hat{g}_{t,k}(j)-S_{t}(j)|\leq \Delta^\prime, \forall j\in [d]$ then 
 \[\left|\sum_{k\in \cC_2} \tilde{g}_{t,k}(j)-S_t(j)\right|\leq \Delta^\prime, \ 1\leq j\leq d.\]
 \end{prop}
 
Each of these $\tilde{g}_{t,k}$s
are then rotated to give $\mathbf{R}\tilde{g}_{t,k}$, each of whose coordinate $\mathbf{R}\tilde{g}_{t,k}(j)$ is encoded using a \emph{Modulo Quantizer} (MQ) $\Qenc_{\tt M}$ described in Algorithm \ref{a:E_MCQ}.  Denote the encoded output by $\Qenc_{\tt M}(\mathbf{R}\tilde{g}_{t,k}(j))\in \{0,\dots, M-1\},$
%\[\varphi_k(\tilde{g}_{t,k})=(\Qenc_{\tt M}(\mathbf{R}\tilde{g}_{t,k}(1)), \dots, \Qenc_{\tt M}(\mathbf{R}\tilde{g}_{t,k}(d))).\]
it can be expressed using at most $\log M$ bits.

\begin{figure}[ht]
\centering
\begin{tikzpicture}[scale=1, every node/.style={scale=1}]
\node[draw,text width= 8 cm, text height=,] {%       
\begin{varwidth}{\linewidth}
            
            \algrenewcommand\algorithmicindent{0.7em}
\begin{algorithmic}[1]
\vspace{-0.5cm}
\Require Input $ x\in \R$, Parameters $M$ and $\Delta^{\prime}$
\State $\eps=5\Delta^{\prime}/ M$
\State $z_u = \ceil{x/\eps}$,  $z_l = \floor{x/\eps}$
  

 \State  
     $
      {\tilde{z}} =
\begin{cases}
z_u, \quad w.p. ~ x/\eps - z_l
 \\ z_l,  \quad w.p. ~  
  z_u-x/\eps
\end{cases}
$
   
 \State \textbf{Output:} $\Qenc_{\tt M}(x)=\tilde{z} \text{ mod } M$
\end{algorithmic}  
\end{varwidth}};
 \end{tikzpicture}
 
 \renewcommand{\figurename}{Algorithm}
 \caption{Encoder  $\Qenc_{\tt M}(x)$ of MQ}\label{a:E_MCQ}
 \end{figure}
 
\paragraph{Mapping to ASK}
We follow an approach similar to the creation of side information.
 In every iteration, the scheme communicates the entire gradient uses in one channel use. In particular, for the same parameter $p\leq d$ as earlier,  each client $k\in \cC_2$ first uniformly samples a set $\mathcal{D}_t\subseteq [d]$ of cardinality $p$. The sampling is done by using the public randomness shared between the clients in $\cC_2$ and the server. Only the coordinates indexed in $\mathcal{D}_t$ are sent after MQ encoding.
Note that overall precision required for each client in every channel-use is $p\log M,$ which can be mapped uniquely to an integer in $\mathcal{A}_2:=\{0,\dots, M^p-1\}.$ 
Denote this integer by $I_{k}\in \mathcal{A}_2$ for client $k\in \cC_2$.
For communication, we consider the same ASK code $\mathcal{B}$ in \eqref{e:ASK} with
% $[-\sqrt{P},\sqrt{ P}]$ with the following $2^r$-constellation points
%\begin{align}\label{e:ASK}
%\left\{-\sqrt{P} +\frac{(i-1)\cdot 2\sqrt{P}}{2^r-1}\colon i \in [2^r] \right\},
%\end{align}
$r=p\log M$. 
Specifically, for client $k\in \cC_2,$ the quantization 
point $I_{k}\in \mathcal{A}_2$ gets mapped to a unique codeword in $\mathcal{B}$ via the mapping $\zeta(I_{k})$ as defined earlier. We call this is $\varphi_k(\hat{g}_{t,k})=\zeta(I_k).$
%and map $i$th client output vector $\varphi_i(\tilde{g}_{t,i}).$ Denote by $\zeta:\{0,...,M-1\}^d\to [-\sqrt{P}, \sqrt{P}]$ the mapping between $\varphi(\tilde{g}_{t,i})$ and $2^r$-ASK code.

All the clients communicate over a MAC channel via \eqref{e:Gaussian_channel_M}. Since $\ell=1$ for every query, the algorithm receives the output $Y_{t, \MAC}\in \R$ is given by 
\[Y_{t,\MAC}=\sum_{k\in \cC_2} \varphi_k(\hat{g}_{t,k})+W_t.\]
\paragraph{Successive cancellation Decoding}
At the algorithm's end, the decoder $\psi$ primarily consists of a minimum-distance decoder,  an inverse mapping $\Omega,$ a MQ decoder $\Qdec_{\tt M}$ described below.

\begin{enumerate}
\item Each $Y_{t,\MAC}$ is first fed into a minimum-distance (MD) decoder that locates the nearest possible ASK codeword in $[-\frac{K}{2}\sqrt{P}, \frac{K}{2}\sqrt{P}]$. Denote the decoded output by $\hat{Y}_{t,\mathtt{MD}}$,
%Note that there exist a one-to-one mapping between the decoded codeword to $$
it is then passed through a inverse mapping $\Omega:[-\frac{K}{2}\sqrt{P}, \frac{K}{2}\sqrt{P}]\to \{0,\dots, (K/2)(M^p-1)\}$ given by $\Omega(x)=\frac{x+(K/2)\sqrt{P}}{2\sqrt{P}/(2^r-1)}.$

\item Note that every output $\Omega(\hat{Y}_{t,\mathtt{MD}})$ can be expressed as 
\[\Omega(\hat{Y}_{t,\mathtt{MD}})=\lambda_{1}+M \lambda_{2}+\dots+M^{p-1} \lambda_{p},\] where %\footnote{Under perfect decoding, $\lambda_{ji}=\sum_{i=1}^KI_{ji.$}
$\lambda_{i}\in \{0,\dots, (K/2)(M-1)\},  i\in [p].$

\item We then follow the successive-cancellation approach to recover each $\lambda_{i} \mod M.$ In particular,  we use the following recursion
\[\hat{\lambda}_{i} \mod M=\frac{\Omega(\hat{Y}_{t,\mathtt{MD}})-\hat{\lambda}_{1}-\dots-M^{i-2}\hat{\lambda}_{i-1}}{M^{i-1}}\mod v, \ 1\leq i\leq p,\]
which requires the knowledge of previously decoded $\{\hat{\lambda}_{k}\}_{k=1}^{i-1}.$ To decode these $\lambda_{k}$ from $\hat{\lambda}_{k}\mod M,$ we follow the procedure $\Qdec_{\tt M}(\hat{\lambda}_{k}\mod M, \mathbf{R}S_t(i))$ described in Algorithm \ref{a:D_MCQ} and form it as
\[\hat{\lambda}_i=\frac{1}{\epsilon}\Qdec_{\tt M}(\hat{\lambda}_i{\mod M}, \mathbf{R}y(i)),  \qquad i\in \mathcal{D}_t.\]

Note that the algorithm make use of the side information $S_t$ only for the sampled coordinates in $\mathcal{D}_t.$ Other coordinates are set to the corresponding coordinate of side information.

The final estimate used by the algorithm is given by
\[\psi(Y_{t,\MAC})=\mathbf{R}^{-1}\left[\frac{d}{p}\sum_{i\in D_t} (\epsilon\hat{\lambda}_i-\mathbf{R}S_t(i))e_i+\mathbf{R}S_t.\right]\]
\end{enumerate}

%%%% the side information constructed, i.e.,  $S_t=\psi(Y_{t,\MAC})$, and is given by 
%%%%\[\psi(Y_{t,\MAC})((j-1)p+i)=-B+\hat{\lambda}_{ji}\cdot \frac{4B}{K(v-1)}, \ 1\leq j\leq d/p, 1\leq i\leq p.\] 
%%%%\end{enumerate}
%%%%
%%%%
%%%%\begin{enumerate}
%%%%\item The channel output $Y_{t,\MAC}$ is fed into a minimum-distance (MD) decoder that locates the nearest possible ASK codeword in $[-K\sqrt{P}, K\sqrt{P}]$. Denote the decoded output by $\hat{Y}_{t,\mathtt{MD}}$,
%%%%%Note that there exist a one-to-one mapping between the decoded codeword to $$
%%%%it is then passed through the mapping $\Omega$ given by 
%%%%\[\Omega(\hat{Y}_{t,\mathtt{MD}})=\frac{\hat{Y}_{t,\mathtt{MD}}+K\sqrt{P}}{2\sqrt{P}/(2^r-1)}.\]
%%%%\item Note that every output $\Omega(\hat{Y}_{t,\mathtt{MD}})$ can be expressed as 
%%%%\[\Omega(\hat{Y}_{t,\mathtt{MD}})=\lambda_1+M \lambda_2+\dots+M^{d-1} \lambda_d,\] where\footnote{Under perfect decoding, $\lambda_j=\sum_{i=1}^K\Qenc_{\tt M}(\mathbf{R}\tilde{g}_{t,i}(j)).$}
%%%%$\lambda_j\in \{0,\dots, K(M-1)\}, j\in [d].$
%%%%\begin{prop}
%%%%It suffices to recover ${\lambda_j\mod M}, 1\leq j\leq d.$
%%%%\end{prop}
%%%%\noindent We therefore follow the successive-cancellation approach to recover each $\lambda_j \mod M.$ In particular,  we use the following recursion
%%%%\[\hat{\lambda}_j \mod M=\frac{\Omega(\hat{Y}_{t,\mathtt{MD}})-\hat{\lambda}_1-\dots-M^{j-2}\hat{\lambda}_{j-1}}{M^{j-1}}\mod M, \qquad 1\leq j\leq d,\]
%%%%which requires the knowledge of previously decoded $\{\hat{\lambda}_i\}_{i=1}^{j-1}.$ Each of these $\hat{\lambda}_i$ are decoded using the decoder of MQ $\Qdec_{\tt M}$ described in Algorithm \ref{a:D_MCQ} and is given by 
%%%%\[\hat{\lambda}_i=\frac{1}{\epsilon}\Qdec_{\tt M}(\hat{\lambda}_i{\mod M}, \mathbf{R}y(i)), i\in \{0,...,j-1\}.\]
%%%%%we do $\Qdec_{\tt M}(w_j, y_j), \forall j,$ where
%%%%\end{enumerate}
%%%% \begin{figure}[ht]
%%%%\centering
%%%%\begin{tikzpicture}[scale=1, every node/.style={scale=1}]
%%%%\node[draw, text width= 8 cm, text height=,] {%       
%%%%\begin{varwidth}{\linewidth}
%%%%            
%%%%            \algrenewcommand\algorithmicindent{0.7em}
%%%% \renewcommand{\thealgorithm}{}
%%%%\begin{algorithmic}[1]
%%%%  \Require Input $w \in \{0, \ldots, M-1\}$, $y \in \R$
%%%%   \State Set $\hat{z}= \arg\min \{ |(zM +w)\cdot \eps -y| \colon z \in \Z\} $
%%%%    \State \textbf{Output:} $\Qdec_{\tt M}(w, y)=(\hat{z}M+w)\eps$\label{step:output_coordinate}
%%%%\end{algorithmic}
%%%%\end{varwidth}};
%%%% \end{tikzpicture}
%%%% 
%%%% \renewcommand{\figurename}{Algorithm}
%%%% \caption{Decoder $\Qdec_{\tt M}(w, y)$ of MQ}\label{a:D_MCQ}
%%%% \end{figure}
%%%%%\paragraph{Construction of side-information $y$}
%%%%%\textbf{Idea 1} The side information is generated by implementing $S(\mathbf{R}, \{\hat{g}_{t,i}\}_{i\in [2K]\setminus [K]}, \frac{B^2}{d}, \mathbf{0}_d).$\\
%%%%%\textbf{Idea 2} Use CUQ from the other paper.

\paragraph{Analysis}
In every iteration,  the construction of side information from the clients in $\cC_1$ require $d/p$ channel uses and 
communicating the gradients from clients in $\cC_2$ require only one channel use. As a result, we can have atmost $N/(d/p+1)$ queries.

For the minimum-distance decoder,  denote by $A_N$ the event where all the ASK codewords
sent over MAC in $N$ channel uses 
are decoded correctly by the algorithm and by $A_N^c$ its complement, i.e.,
$A_N^c := \cup_{t=1}^{N} \{|W_{t}| \geq 2\sqrt{P}/(2^r-1)\}$,
where $W_{t}\sim \cN(0,\sigma_m^2)$.
We have
\begin{align*}
\E{f(x_N)-f(x^\ast )}&=\E{(f(x_N)-f(x^\ast))\mid A_{N}}\cdot \bPr{A_{N}}+\E{(f(x_T)-f(x^\ast))\mid A_{N}^c}\cdot \bPr{A_{N}^c}\\
&\leq \E{(f(x_N)-f(x^\ast))\mid A_{N}}+DB\cdot \bPr{A_{N}^c}. \numberthis \label{e:ubs}
\end{align*}
As $\bPr{A_N^c} \leq N\exp\left( -\frac{2\SNR}{(2^r-1)^2}\right)$,  setting $r=\log\left( \sqrt{\frac{2\SNR}{\ln K+3\ln N}}+1\right)$ gives $\bPr{A_N^c}\leq \frac{1}{K\sqrt{N}}.$ 
Using Lemma \ref{thm1}, the first term on the right-side can be bounded as 
\begin{align*}
\E{(f(x_N)-f(x^\ast))\mid A_{N}}&\leq \sqrt{2}D\left(\frac{\alpha(\pi, \bar{\varphi}, \psi)}{\sqrt{N/\ell}}+\beta(\pi, \bar{\varphi}, \psi)\cdot\left(1+\frac{1}{\alpha(\pi,\bar{\varphi}, \psi)\sqrt{2N/\ell}}\right)\right)+\frac{LD^2}{2N/\ell}.
\end{align*}
\newer{Note that under perfect decoding, $\hat{Y}_{t,\mathtt{MD}}=\sum_{k\in \cC_2}\zeta(I_k).$ Accordingly, $\Omega(\hat{Y}_{t,\mathtt{MD}})=\sum_{k\in \cC_2}\Qenc_{\tt M}(\mathbf{R}\tilde{g}_{t,k}(1))+\dots+M^{p-1}\sum_{k\in \cC_2}\Qenc_{\tt M}(\mathbf{R}\tilde{g}_{t,k}(p)).$ Thus, we need $M$ sufficiently large so that $\lambda_i=\sum_{k\in \cC_2}\Qenc_{\tt M}(\mathbf{R}\tilde{g}_{t,k}(i)), \forall i\in \mathcal{D}_t$, which requires us to characterise $\|\|$ }


\subparagraph{Closeness of side information}
\begin{lem}
For all $x_t\in \X$ and $i\in [d],$
\[\left\|\sum_{k\in \cC_1}Q_v(\tilde{g}_{t,k}(i))-\nabla f(x_t)(i)\right\|_{\psi_2}^2\leq \sigma^{\prime 2},\]
where $\sigma^{\prime 2}:=\frac{8\sigma^2}{K\ln 2}.$
\end{lem}
\begin{proof}
From the construction of side information, we have
\[\left\|Q_v(\tilde{g}_{t,k}(i))-\tilde{g}_{t,k}(i)\right\|_{\psi_2}^2\leq \frac{16B^2}{(\ln 2)K^2(v-1)^2}.\]
Using the concentration bounds for sum of the independent sub-gaussian rvs ($cf.$ \cite[Prop. 2.6.1]{vershynin2018high}), we have for some absolute constant $C>0$
\[\left\|\sum_{k\in \cC_1}Q_v(\tilde{g}_{t,k}(i))-\sum_{k\in \cC_1}\tilde{g}_{t,k}(i)\right\|_{\psi_2}^2\leq \frac{8CB^2}{(\ln 2)K(v-1)^2}.\] Further, from \eqref{e:mean_square}, we have $\left\|\sum_{k\in \cC_1}\tilde{g}_{t,k}(i)-\nabla f(x_t)(i)\right\|_{\psi_2}^2\leq \frac{2\sigma^2}{K\ln 2}.$ 
Using the inequality: $(a+b)^2\leq a^2+b^2,$ we have 
\[\left\|\sum_{k\in \cC_1}Q_v(\tilde{g}_{t,k}(i))-\nabla f(x_t)(i)\right\|_{\psi_2}^2\leq \frac{4\sigma^2}{K\ln 2}+ \frac{16CB^2}{(\ln 2)K(v-1)^2}.\]
Setting $v=\max\{2(1+B), 1+\frac{2B\sqrt{C}}{\sigma},\}$ the right hand side above can be upper bounded by $ \frac{8\sigma^2}{K\ln 2}.$
\end{proof}

\subparagraph{Rotation induces subgaussianity, preserves the closeness:} Under the perfect decoding, the side information is equal to sum of quantized coordinates, i.e, $S_t(j)=\sum_{k\in \cC_1}Q_v(\tilde{g}_{t,k}(j)), \ j\in [d]$ in the above lemma. Consequently,  we have the following lemma to motivate the idea of rotation.
\begin{lem}\label{l:rot_si}
For all $x_t\in \R^d$ and $i\in [d],$ we have
\[\mathbb{P}(|\mathbf{R}S_t(i)-\mathbf{R}\nabla f(x_t)(i)|\geq t)\leq 2e^{-c\min\{t^2/\sigma^{\prime 2}, t\sqrt{d}/\sigma^\prime\}},\]
where $c>0$ is an absolute constant.
\end{lem}
\begin{proof}
Note that $\mathbf{R}S_t(i)-\mathbf{R}\nabla f(x_t)(i)=\sum_{j\in[d]}U_{ij}V_j,$ where $\|U_{ij}\|_{\psi_2}\leq \frac{1}{\sqrt{d}\ln 2}$ and $\|V_j\|_{\psi_2}\leq \sigma^{\prime}.$
Using the fact that product of two sub-gaussian rvs sub-exponential rv ($cf.$ \cite[Lemma 2.7.7]{vershynin2018high}),  we have
\[\|U_{ij}V_j\|_{\psi_1}\leq \frac{\sigma^{\prime}}{(\ln 2)\sqrt{d}}.\]
Using the Bernstein inequality (\cite[Lemma 2.8.1]{vershynin2018high}) for the sum of independent mean-zero sub-exponential rvs, the proof is completed.
\end{proof}
Further, using the Lemma \ref{l:rot}, we have
\[\mathbb{P}(|\mathbf{R}\nabla f(x_t)(i)-\sum_{k\in \cC_2}\mathbf{R}\tilde{g}_{t,k}(i)|\geq t)\leq 2e^{-dKt^2(\ln 2)/(4\sigma^2)}.\]


and combining with Lemma \ref{l:rot_si} via union bound, we have
\[\mathbb{P}(|\mathbf{R}S_t(i)-\sum_{k\in \cC_2}\mathbf{R}\tilde{g}_{t,k}(i)|\geq t)\leq 2e^{-c\min\{t^2/(4\sigma^{\prime 2}), t\sqrt{d}/(2\sigma^\prime)\}}+2e^{-dKt^2(\ln 2)/(8\sigma^2)}.\]

==> result__Shubham_Jha_s_conflicted_copy_2022-12-16_.tex <==
\section{ A digital communication scheme for over-the-air optimization}\label{s:results}

In this section, we present our main result: a digital communication scheme that, when combined with PSGD, will almost match the lower bound in  Theorem \ref{t:OTAlb}. We omit the subscript $t$ for convenience. {Our schemes below are ``universal'' in the sense that the clients don’t
require the knowledge of $\sigma$ for the transmission of gradient estimates.}
%Note that for $K=1$ the above exactly matches the lower bound in \cite{JMT22jsait}.
%To show the above, we use 0-smooth affine functions as difficult functions and consider Bernoulli oracles, similar to \cite{JMT22jsait}.
%The key step involves the decomposition of Gaussian MAC into sum of independent white Gaussian channels and using a bound on achievable sum rate \cite{CovTho06}.
%We skip the proof details here for brevity.
\subsection{Warm-up scheme {\tt UQ-OTA}}
For ease of presentation, we first present a warm-up scheme based on uniform quantization. We will build on the components present in this scheme to build our final digital scheme.
\paragraph{Uniform quantization }
 Each client $k$ first divides the gradient estimate $\hat{g}_{k}$ by number of clients $K$ to form $\tilde{g}_{k}$ and quantizes it using an unbiased $v$-level {\em coordinate-wise uniform quantizer} $v$\texttt{-CUQ}.
The $v$\texttt{-CUQ} takes $i$th coordinate $\tilde{g}_{k}(i)\in [-\frac{B}{K},\frac{B}{K}]$ as input and outputs $z_{k,i}\in \{0,...,v-1\}$ by the following rule:
\begin{align*}\label{e:CUQ}
z_{k,i}= 
\begin{cases}  
\ceil{\frac{(v-1)(K\tilde{g}_{k}(i)+B)}{2B}}, \text{ w.p. }  \frac{\tilde{g}_{k}(i) - \floor{\frac{\tilde{g}_{k}(i)K(v-1)}{2B}}}{2B/(K(v-1))}\\
\vspace{2pt}
 \floor{\frac{(v-1)(K\tilde{g}_{k}(i)+B)}{2B}}, \text{ w.p. } \frac{\ceil{\frac{\tilde{g}_{k}(i)K(v-1)}{2B}} - \tilde{g}_{k}(i)}{2B/(K(v-1))}
\end{cases}.
\end{align*}
Note that the $z_{k,i}$ suffices to form an unbiased estimate of $\tilde{g}_{k}(i)$. Thus, client $k$ transmit $z_{k,i}$s over MAC. This is done by first encoding them onto a lattice and then, modulating them as ASK codewords. 
Define $\mathtt{Q}_k\coloneqq \{z_{k,i}:i\in [d]\}$ as the quantized output for client $k$, we refer to this procedure as $\mathcal{M}({\tt Q}_{k},v,p)$ with parameters $v$ and $p$ to be specified later.
\paragraph{Lattice encoding and ASK modulation using $\mathcal{M}({\tt Q}_{k},v,p)$}
 For some parameter\footnote{We assume $p$ divides $d$.} $p\leq d$, the set of coordinates $[d]$ is equally partitioned into $d/p$ blocks. The $j$th block is given by $\mathcal{B}_j:=\{(j-1)p+1, \dots, (j-1)p+p\}, j{\in} [d/p].$ For each $\mathcal{B}_j$, the corresponding quantized values are mapped onto a lattice generated by bases $\{w^0,...,w^{p-1}\}$. In particular, the lattice point $\tau_{k,j}$ is given by 
 %the corresponding entries $z_k(\mathcal{B}_j) \in \{0,...,v-1\}^p$
%using a function defined below.
%  \begin{defn}
%A {\em pre-processing function} is a map $\tau:\{0,...,v-1\}^{p}\to \mathbb{Z}$ that takes an input vector $z$ and outputs an integer lattice point generated by $\{w^0,...,w^{p-1}\}$ as
%
\begin{align}\label{e:tau}
    \tau_{k,j}= w^0{\tt Q}_k(\mathcal{B}_j(1))+\dots+w^{p-1}{\tt Q}_k(\mathcal{B}_j(p)),
\end{align}
for $w{=}K(v-1)+1$. For the ease of description, we abbreviate \eqref{e:tau} as $\tau_{k,j}=({\tt Q}_k(\mathcal{B}_j(1)),..., {\tt Q}_k(\mathcal{B}_j(p)))_w$.
\snote{The above shorthand simplifies the decoding description.}

 To satisfy the power constraints of MAC, we then modulate each $\tau_{k,j}$ to $[-\sqrt{P}, \sqrt{P}]$ using an ASK code. 
\begin{defn}\label{d:ASK_codes}
  A code is an
  %\footnote{For simplicity, we have considered AWGN channel for transmission.
 %In many practical communication systems, a two-dimensional signal space is available through the in-phase
 %and quadrature-phase components. For these systems, our results for ASK code
%continue to hold with a QAM or QPSK constellation-based code.} 
\emph{Amplitude Shift Keying (ASK)
  code} satisfying the average power constraint \eqref{e:Power_constraint} if the range $\mathcal{A}$
of the encoder mapping is given by
\begin{align}\label{e:ASK}
\mathcal{A}:=\left\{-\sqrt{P} +(i-1)\cdot \frac{2\sqrt{P}}{r-1}\colon i \in [r] \right\},
\end{align}
for some $r\in \N$.
Note that
this is a code of length $1$.
\end{defn}
Since each $\tau_{k,j}$ takes values in $\{0,...,\frac{w^{p}-1}{K}\}$, we use $r=\frac{w^p-1}{K}+1$ in $\mathcal{A}$, and $\mathcal{A}(\tau_{k,j}+1)$ forms $j$th channel input $\varphi_k(j)$. Accordingly, the server obtains channel output $Y\in \R^{d/p}$ \eqref{e:Gaussian_channel_M}. 
\paragraph{Lattice decoding at server $\mathcal{L}(Y,v,p)$} 
Note that it suffices to recover the sum $\bar{z}=\sum_kz_k$, instead of individual $z_k$s, to determine an unbiased estimate of sum of clients' inputs.

Towards that,  each coordinate $Y(j)$ is fed into a coordinate-wise minimum-distance (MD) decoder, thereby, locating the nearest possible point $\hat{Y}(j)$ in $\{-K\sqrt{P}+\frac{2(i-1)\sqrt{P}}{r-1}:i\in [r]\}$.
Using the one-to-one correspondence, the decoded point $\hat{Y}(j)$ is then mapped back to the lattice generated using $\{w^0,...,w^{p-1}\}$ to decode the sum of transmitted lattice points $\sum_k\tau_{k,j}$. 
Denote by $\hat{\bar{\tau}}_j$ the decoded lattice point is given by \[\hat{\bar{\tau}}_j=\frac{\hat{Y}(j)+K\sqrt{P}}{2\sqrt{P}/(r-1)}, \ j \in [d/p].\]  
It is easy to see that $\hat{\bar{\tau}}_j=(\lambda(\mathcal{B}_j(1)), ..., \lambda(\mathcal{B}_j(p)))_w$ for some vector  $\lambda\in \{0,...,K(v-1)\}^d$. Therefore, to recover the desired sum,  the server uses a {\em modulo-lattice decoder} for each $\mathcal{B}_j, j\in [d/p]$, that successively outputs the coordinates of $\lambda$. In particular $\forall i \in [p]$,
\begin{align}\label{e:SC_dec}
    \lambda(\mathcal{B}_j(i))=\frac{\hat{\bar{\tau}}-\lambda(\mathcal{B}_j(1))...-w^{i-2}\lambda(\mathcal{B}_j(i-1))}{w^{i-1}}\mod w.
\end{align}
Note that such recovery is possible with the current choice of $w$.
The value $\lambda$ obtained above is finally used to form $\psi(Y)$ to be used in Alg.  \ref{a:SGD_Q} as
\begin{align}\label{e:est_CUQ}
\psi(Y)=-B+\lambda\cdot \frac{2B}{K(v-1)}.
\end{align}
\begin{thm}\label{t:CUQ}
Let $\pi$ be the optimization algorithm described in Algorithm \ref{a:SGD_Q} where $\psi(Y)$ is obtained in \eqref{e:est_CUQ} with $v=\sqrt{d}+1$. 
Then,
  for a universal constant $c_1$ and integers $p,K$ such that ${d \geq p \geq 1}$ and $K\geq B^2/\sigma^2$, we have
\begin{align*}
\sup_{(f,\cC)\in \cO}\cE(f, \clientset, \pi, Q) &\leq  \frac{c_1DB}{\sqrt{KN}}\sqrt{\frac{d}{p}}+\frac{LD^2d}{2Np},
\end{align*}
where $p=\floor{\frac{\log\left(1+\sqrt{\frac{2K\SNR}{\ln(KN^{1.5})}}\right)}{\log (Kd)}}$.
\end{thm}
%\newest{\begin{rem}We remark that the above scheme {\tt UQ-OTA} is \emph{universal} in the sense that the clients don't require the knowledge of $\sigma$ for the transmission of gradient estimates.\end{rem}}
%\mnote{Reminder: $p$, $v$ should be independent of $\sigma$. This will ensure we get $DB/\sqrt{T}$ convergence rate here and our quantizers at the clients are independent of $\sigma$. Right a remark saying this is universal compression.}
%\snote{Since both schemes are universal, added a line in the beginning of this section )but not as a remark).}
\begin{rem}[Size of codebook grows with SNR]\label{r:1}
 We remark that the size of ASK codebook $\mathcal{A}$ used for MAC transmission grows with the operating $\SNR$ as $r\approx \min (\sqrt{d}+1,\floor{1+\sqrt{2\SNR/(K\ln(KN^{1.5}))}})$.
%\snote{$r\geq \sqrt{d}+1$ due to $p=1$ in $w^d-1=K(r-1)$.}
\end{rem}
\begin{rem}[Sub-optimality of {\tt UQ-OTA}]
    For $\SNR\geq \frac{\ln(KN^{1.5})(w^{d}-1)^2}{2K}$, the {\tt UQ-OTA} incur a $(B/\sigma)\sqrt{\log(Kd)}$ factor slowdown in convergence rate compared to that of centralized setting. 
\end{rem}
%From the remarks above, note that the factor $B\sqrt{\log(Kd)}$ can still cause slowdown in performance for large $d$.
%In addition, the sub-optimal factor on dimension  may still be concern.
We now present the main digital scheme that reduces this dependence to $\sqrt{B\sigma}\log(K\ln(KN))$ and is almost optimal.
%\input{wz1}
\input{wz2}


==> wz1.tex <==
\subsection{A Wyner-Ziv approach}
In each iteration $t$, the clients in $\cC_1$ construct the side information at the server and then the remaining clients in $\cC_2$ exploit this information to form a Wyner-Ziv type estimate of $\nabla f(x_t)$ at the server, where $\cC_1:=C_1, \dots, C_{K/2}, \cC_2:=\cC\setminus \cC_1.$
\subsubsection{Side information construction}
The $K/2$ clients in $\cC_1$ use CUQ and modulation technique described above to construct the side information. Denote by $S_t$,  constructing the side information requires $d/p_1$ channel uses.
\subsubsection{The Wyner-Ziv estimate}
The side-information constructed by the clients in $\cC_1$ to form the actual gradient estimate at the server.  Specifically, the clients in $\cC_2$ incorporate the available side information at the server and communicate the gradient estimates using DAQ quantizer from \cite[Section 4.2]{mayekar2021wyner}. 
The DAQ builds on the correlated sampling idea using shared randomness and gives the unbiased estimate for $x$ with side information $y.$ In particular, $\forall i\in [d],$ the estimate is
\begin{align}\label{e:daq}
\hat{X}(i)=2M\left(\mathbbm{1}_{\{U(i)\leq x(i)\}}-\mathbbm{1}_{\{U(i)\leq y(i)\}}\right)+y(i), 
\end{align}
provided $x(i),y(i)\in [-M, M]$ and $U(i)\sim \mathtt{Unif}[-M,M].$ 

 In our setting, the clients in $\cC_2$ uses DAQ with $S_t$ being the side information at server.
Each client ${k\in \cC_2}$ forms the vector $\tilde{g}_{t,k}=\frac{\hat{g}_{t,k}}{K/2}$ and draws $U_{t,k}(i)\sim \mathtt{Unif}[-2B/K, 2B/K], \forall i\in [d],$ using shared randomness. 
Further, $\tilde{g}_{t,k}$ is quantized using the popular {\em 1-bit stochastic quantizer} described below.
\paragraph{1-bit quantization} Quantize $\tilde{g}_{t,k}$ as
\[\Qenc_{t,k}(i):=\mathbbm{1}_{\{U_{t,k}(i)\leq \tilde{g}_{t,k}(i)\}}, \ i\in [d].\]
Similar to the side information construction, these quantized values are next mapped to ASK codes for transmission.
\paragraph{Mapping to ASK} For a parameter $p_2\leq d,$ the set of coordinates $[d]$ is partitioned into blocks of size $p_2$ given by $\mathcal{B}_j:=\{(j-1)p_2+1, \dots, \min(d,(j-1)p_2+p_2)\}, j\in [d/p_2].$ For each $\mathcal{B}_j,$ the corresponding bit values $\{\Qenc_{t,k}(i)\}_{i\in \mathcal{B}_j}$ are represented using bases $w_2^0,\dots, w_2^{p_2-1}$ as
\[\tau_{t,k}^{\mathtt{WZ}}(j){:=}w_2^0\cdot \Qenc_{t,k}(\mathcal{B}_j(1))+\dots+w_2^{p_2-1}\cdot \Qenc_{t,k}(\mathcal{B}_j(p_2)),\]
where $w_2:=K/2+1.$ 

Now, each $\tau_{t,k}^{\mathtt{WZ}}(j)$ is mapped to a $2^r$-ASK code in $\mathcal{A}$ \eqref{e:ASK} with $r=p_2\log w_2$ 
and the mapping is given by \[\varphi_{k}(\hat{g}_{t,k})(j)=-\sqrt{P}+\frac{\tau_{t,k}^{\mathtt{WZ}}(j)2\sqrt{P}}{2^r-1}, k\in \cC_2, j\in [d/p_2].\] 
%This requires $\ell=d/p_2$ channel uses per iteration.
Denote
by $Y_{t,\mathtt{WZ}}\in \R^\ell$ the $d/p_2$-dimensional output obtained via \eqref{e:Gaussian_channel_M}. 
\paragraph{Decoding} At the server,  the decoder $\psi$ does the following:
\begin{enumerate}
\item Each coordinate $Y_{t,\mathtt{WZ}}(i)$ is fed into a MD decoder locating the nearest ASK codeword in $\hat{Y}_{t,\mathtt{WZ}}(j)\in [-\frac{K\sqrt{P}}{2}, \frac{K\sqrt{P}}{2}]$.

 \item The $\hat{Y}_{t,\mathtt{WZ}}$ is then mapped back to the lattice generated by the bases $\{w_2^{i}\}_{i=0}^{p_2-1}$ via 
mapping\footnote{Under perfect decoding, $\Omega(\hat{Y}_{t,\mathtt{WZ}}(j)){=}\sum_{k\in \cC_2}\tau_{t,k}^{\mathtt{WZ}}(j), \lambda_{ji}=\sum_{k\in \cC_2}\Qenc_{t,k}(\mathcal{B}_j(i)).$.}
$\Omega(x)=\frac{x+(K/2)\sqrt{P}}{2\sqrt{P}/(2^r-1)}.$
Note that every output $\Omega(\hat{Y}_{t,\mathtt{WZ}}(j))$ can be expressed as 
\[\Omega(\hat{Y}_{t,\mathtt{WZ}}(j))=w_2^0\lambda_{j1}+\dots+w_2^{p_2-1} \lambda_{jp_2},\ j\in [d/p_2],\] for some
$\lambda_{ji}\in \{0,\dots, K/2\},  i\in [p_2].$

\item We then follow the successive-cancellation approach to recover each $\lambda_{ji}.$ In particular,  we use the following recursion for $1\leq j\leq d/p_2,1\leq i\leq p_2,$
\[\lambda_{ji}=\frac{\Omega(\hat{Y}_{t,\mathtt{WZ}}(j))-\lambda_{j1}-\dots-w_2^{i-2}\lambda_{j(i-1)}}{w_2^{i-1}}\text{ mod } w_2.\]
\end{enumerate}
%which requires the knowledge of previously decoded $\{\hat{\lambda}_{jk}\}_{k=1}^{i-1}.$ To decode these $\lambda_{jk}$ from $\hat{\lambda}_{jk}\mod v,$ we follow the procedure $\Qdec_{\tt M}(\hat{\lambda}_{jk}\mod v)$ described in Algorithm \ref{a:D_MCQ}.
For $j\in [d/p_2],  i\in [p_2],$ the final WZ estimate  is given by
\begin{align*}
\psi(Y_{t,\mathtt{WZ}})(\mathcal{B}_j(i))&{=}\frac{4B}{K}\left(\lambda_{ji}-\sum_{k\in \cC_2}\mathbbm{1}_{\{U_{t,k}(\mathcal{B}_j(i))\leq \frac{S_t(\mathcal{B}_j(i))}{K/2}\}}\right)\\&\qquad+S_t(\mathcal{B}_j(i)).
\end{align*} 
We next characterise the performance of this WZ scheme.
\begin{thm}\label{t:UQSGD}
Fix $v=1+\sqrt{d}$ for the CUQ $Q_v.$
 Let $\pi$ be the optimization algorithm described in Algorithm \ref{a:SGD_Q} where $\psi(Y_{t,\mathtt{WZ}})$ is used to make the PSGD step after the $t$th query. Then,
  for universal constants $c_1$ and $c_2$ and 
 $r=\log(1+\sqrt{\SNR/(K\ln(KN))})$ such that ${d \geq r \geq c_1\log (Kd)}$, we have
\begin{align*}
\sup_{(f,\cC)\in \cO}\cE(f, \clientset, \pi, S) &\leq  \frac{c_2D\sqrt{d\log (Kd)}}{\sqrt{rKN}}\sqrt{\sigma^2 +\rho(B,\sigma,d,K)}\\
&\qquad+\frac{DB}{K\sqrt{N}}
+ \frac{L D^2d\log (Kd)}{2Nr},
\end{align*}
where $\rho(B,\sigma,d,K)=4\sqrt{d}B\sqrt{\frac{4\sigma^2}{K}+\frac{32B^2}{K}+\sigma^2}.$
\end{thm}
\begin{rem}
For $\SNR\gtrapprox 2^{2d}$ and $K\geq B^2/\sigma^2,$ the parameter $\rho\approx B\sigma\sqrt{d}$ and the convergence rate is better than that in Theorem \ref{t:CUQ} for $\sigma$ smaller than $B/\sqrt{d}.$
%reduces to $\frac{c_2 D\sqrt{\log(Kd)}}{\sqrt{KN}}\sqrt{\sigma^2+\sqrt{d}B\sigma}+\frac{LD^2\log(Kd)}{N}$, which 
\end{rem}
